Performance of the ATLAS Trigger System in 2015

During 2015 the ATLAS experiment recorded 3.8 fb$^{-1}$ of proton--proton collision data at a centre-of-mass energy of 13 TeV. The ATLAS trigger system is a crucial component of the experiment, responsible for selecting events of interest at a recording rate of approximately 1 kHz from up to 40 MHz of collisions. This paper presents a short overview of the changes to the trigger and data acquisition systems during the first long shutdown of the LHC and shows the performance of the trigger system and its components based on the 2015 proton--proton collision data.

==> content/outlook.tex <==
Outlook for 2016 data-taking...


